TalkNCE: Improving Active Speaker Detection with Talk-Aware Contrastive Learning

The goal of this work is Active Speaker Detection (ASD), a task to determine whether a person is speaking or not in a series of video frames. Previous works have dealt with the task by exploring network architectures while learning effective representations has been less explored. In this work, we propose TalkNCE, a novel talk-aware contrastive loss. The loss is only applied to part of the full segments where a person on the screen is actually speaking. This encourages the model to learn effective representations through the natural correspondence of speech and facial movements. Our loss can be jointly optimized with the existing objectives for training ASD models without the need for additional supervision or training data. The experiments demonstrate that our loss can be easily integrated into the existing ASD frameworks, improving their performance. Our method achieves state-of-the-art performances on AVA-ActiveSpeaker and ASW datasets.

==> table/table_able_lossposition.tex <==
% \begin{table}[t!]
% \centering
% \caption{Performance evaluation by the position of loss. CA is a cross-attention module for audio-visual fusion.}
% \vspace{0.2cm}
% \label{table3}
% \begin{tabular}{lccc} 
% \Xhline{2\arrayrulewidth}
% \Xhline{0.1pt}  
% Method                   & epoch 10 & epoch 20 & best       \\ 
% \hline
% After CA                 &92.81     & 93.07    & 93.42            \\
% Before CA & \textbf{94.27}    & \textbf{95.47}    & \textbf{95.51}  \\
% \Xhline{2\arrayrulewidth}
% \Xhline{0.1pt}  
% \end{tabular}
% \end{table}

\begin{table}[t!]
\centering
\vspace{0.2cm}
{\small
\begin{tabular}{lc} 
\Xhline{2\arrayrulewidth}
\Xhline{0.1pt}  
Position of our loss               & mAP(\%)$\uparrow$       \\ 
\hline
None (Baseline) & 95.2 \\
After CA           & 93.42            \\
\textbf{Before CA}    & \textbf{95.51}  \\
\Xhline{2\arrayrulewidth}
\Xhline{0.1pt}  
\end{tabular}
}
\caption{Performance evaluation of LoCoNet~\cite{loconet} by the position of TalkNCE loss. CA denotes cross-attention module for audio-visual fusion.}
\label{table_able_lossposition}
\end{table}

==> table/table_able_lossweight.tex <==
\begin{table}[t!]
\centering
\vspace{0.1cm}
\begin{tabular}{lc} 
\Xhline{2\arrayrulewidth}
\Xhline{0.2pt}  
$\lambda$ value               & mAP(\%)$\uparrow$       \\ 
\hline
0.15         & -            \\
\textbf{0.3}           & \textbf{95.51}        \\
0.6    & -  \\
\Xhline{2\arrayrulewidth}
\Xhline{0.1pt}  
\end{tabular}
\caption{Performance evaluation depending on various value of $\lambda$ for loss weight.}
\label{table_able_lossweight}
\end{table}



==> tex/5_Acknowledge.tex <==
\section{Acknowledgements}
\label{ack}


This work is supported by Naver Corporation. We would like to thank  Icksang Han, Bong-Jin Lee, and Hee-Soo Heo for helpful discussions, and Yidi Jiang for the help with re-implementation of ASW experiments.
%~\cite{jiang2023target}.

==> tex/exp_copy.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Datasets}
\label{ssec:exp_datasets}
\newpara{AVA-ActiveSpeaker dataset}~\cite{roth2020ava} is a benchmark for evaluating active speaker detection performance extracted from Hollywood movies. It contains 262 videos that span 38.5 hours, of which 120, 33, and 109 videos are divided into training, validation, and test set respectively. As the videos are from movie films, the dataset includes dubbed videos, and `active' labels are used even though the audio and video are not perfectly synchronized.

\newpara{Active Speakers in the Wild (ASW) dataset}~\cite{lwt} is a dataset derived from the existing audio-only speaker diariazation dataset VoxConverse~\cite{chung2020spot} by randomly selecting 212 videos and exploiting the diarization annotations.
Unlike the AVA-ActiveSpeaker dataset, this dataset excluded dubbed videos to ensure synchronization between lip movements and the speech signal. Videos in the dataset span 30.9 hours in total, and the ratio of the duration of active tracks are 56.7\%, 60.4\%, and 57.0\% for the training, validation, and test set individually. Note that 4 videos cannot be downloaded due to a privacy issue.

\begin{figure}[t!]
\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=7.5cm]{figures/asd_sync_final.pdf}}
\end{minipage}
\caption{Cross modal loss for audio embedding and visual embedding. The loss is applied only to the active section, which is marked as `active', and not applied to the `inactive' section, which is colored in gray. Audio and video pairs colored in blue are positive pairs, which are in sync, and the orange-colored pairs are negative as they are asynchronized.}
\label{fig:res}
%
\end{figure}


\subsection{Implementation details}
\label{ssec:exp_impl}
Models that we reproduced for performance comparison are trained following the details of each model~\cite{loconet,lightASD, talknet}. We train each model end-to-end for 25 epochs using Adam optimizer~\cite{KingBa15} with weight decay. Feature dimension of both audio and visual embeddings are set to 128 for all three models. The value for $\lambda$ was empirically set to 0.3 for LoCoNet to make similar scale with $\mathcal{L}_{av}$. Similarly, $\lambda$ values for other models~\cite{talknet, lightASD} are assigned considering magnitudes with the existing loss.


As a multi-speaker model, outputs of LoCoNet are the predictions of not only target speakers but also context speakers.
Therefore, the original loss is an average of cross entropy loss computed for the prediction of every speaker.
The TalkNCE loss is also applied to audio and visual embeddings of active speaking frames for all speakers.
For the other models such as TalkNet~\cite{talknet} which exploits only one speaker's information, we also follow the training details of each model when the models are trained with the TalkNCE loss. 


\input{table/table1}

\input{table/table2}

\subsection{Performance on AVA-ActiveSpeaker Dataset}
\label{ssec:exp_ava}
Table~\ref{table1} shows the comparison of our method and previous results.
Mean average precision (mAP) is used as an evaluation metric, as in previous works~\cite{loconet, lightASD, talknet, kopuklu2021design}. 
As shown in Table~\ref{table1}, LoCoNet trained with our loss achieves 95.5\% mAP, outperforming the existing state-of-the-art methods.
In Table~\ref{table2}, we also adopt the loss for TalkNet and Light-ASD to examine the generalizability of our loss other than LoCoNet. 
It is evident that our loss increases performances in our reproduced models~\cite{talknet, lightASD}.

%For TalkNet, our loss enhances the best mAP for 0.44\%p in Table~\ref{table2}. 
%For the TalkNet model trained along with our loss, the performance on the earlier epochs were higher than the later epochs of exiting TalkNet. 
%For the LightASD model, the loss has little effect on the rate of performance convergence, but there is no doubt that the loss increases the performance of the reproduced Light-ASD.


%It is evident that our loss increases performances in our reproduced Light-ASD.

%Other than the baseline, we also adopt the loss for TalkNet and Light-ASD. For TalkNet, our loss enhances the best mAP for 0.44\%p in Table~\ref{table2}. \syun{For the TalkNet model trained along with our loss, the performance at earlier epochs are higher than the performance at later epochs of the vanilla TalkNet. For the LightASD model, the loss had little effect on the rate of performance convergence, but there is no doubt that the loss increases the performance of the reproduced Light-ASD.}



\subsection{Performance on ASW Dataset}
\label{ssec:exp_asw}

\input{table/table3}

As denoted in Table~\ref{table3}, our method achieves state-of-the-art results with huge margin for ASW validation and test set on three evaluation metrics: Area under the ROC Curve (AUC), equal error rate (EER), and mAP. Table~\ref{table3} is constructed based on \cite{jiang2023target} and, for fair comparison, we got codes from the author of \cite{jiang2023target} for evaluation on ASW dataset. Our highest performance was obtained by adding $\mathcal{L}_{TalkNCE}$ to LoCoNet model. 
Different from AVA-ActiveSpeaker dataset, ASW dataset does not include dubbed video. This makes our loss more effective in ASW dataset, since our loss is applied to optimize the performance through the audio-visual correspondence.
% There is no dubbed video in ASW dataset different from AVA dataset which involves dubbed videos. Since TalkNCE loss is applied to audio-visual synchronized regions, our loss can press enormous effects on ASW performances.

% val (mAP = 98.81, AUC = 99.34, EER = 3.17 @ epoch22)
% test(mAP = 99.30, AUC = 99.52, EER = 2.99 @ epoch19)

\subsection{Ablation Studies}
\label{ssec:exp_ablation}

\newpara{Weight value of $\mathcal{L}_{TalkNCE}$.}
\jyj{(see comment.)}Table \ref{table4} shows the performance of our TalkNCE loss combined with LoCoNet regarding $\lambda$ values and the position of our loss. 
$\lambda$ values do not have a huge impact on performances. However, 0.3 value gets the highest score and we guess that when we set $\lambda$ to 0.3, our loss and existing $\mathcal{L}_{av}$ become similar in early training steps and can be trained in balance.


\newpara{Position of $\mathcal{L}_{TalkNCE}$.}
As we suppose, our proposed loss is especially effective for refining the embedding before audio-visual fusion as indicated in Table~\ref{table4}. 
When it is inserted after the audio-visual fusion stage, it has a negative effect on performance.
Applying contrastive learning to the attention-weighted features $f_a$ and $f_v$ seems to have a negative influence on performances. \jyj{(see comment.)} Since our TalkNCE loss can refine uni-modality features by giving rich information with frame-level synchronization, our loss is not proper to give a multi-modal guidance to $f_a$ and $f_v$, which have already interacted with each other during the fusion stage. 

\input{table/table4}
%following concatenation operation than cross-attention, even harming the performance of the baseline. 

%so the performance declines. 
%between the relative audio-visual pair 
\input{table/table5} 
\newpara{Choice of positive and negative samples.}
\jyj{(see comment.)}By using the labels for a certain speaker, a sequence of audio and visual embeddings can be divided into `active' and `inactive' regions, as in Fig~\ref{fig:res}. Our proposed method includes only `active' regions of both embeddings for $\mathcal{L}_{TalkNCE}$, and Table~\ref{table5} shows results obtained by different choices of samples. 
In Table~\ref{table5}, `active' means that $\mathcal{L}_{TalkNCE}$ is calculated for only active regions for the embedding, and `all' means that $\mathcal{L}_{TalkNCE}$ is calculated by utilizing all regions regardless of activeness. This experiment explains that our proposed loss learns from the synchronization of audio and video.
%
As shown in the table, utilizing inactive frames of audio embedding does not enhance performance. As the audio in inactive region includes sounds irrelevant to the speaker's speech, it hinders the learning of audio-visual correspondence.
%
Visual information from inactive regions include silent faces, which can be classified as a negative pair with audio from active regions. However, inactive video regions also include non-speaking lip movements, which can confuse the learning of accurate synchronization of audio and video.
Therefore the performance obtained by all visual embedding is still lower than the combination of active regions.
%
Utilizing the full segment increases the total number of samples for our loss, but silent faces and irrelevant audio are paired as positive, which is not desirable to focus on the synchronization of two modalities. Therefore, this approach degrades performance, and we suppose that our loss can optimize the model when the accurate selection of pairs is guaranteed.

% Active frame region in which audio and visual features are synchronized as `active' in Fig~\ref{fig:res}. The last row in Table~\ref{table4} shows the highest score in AVA-ActiveSpeaker validation dataset. The other rows are results of the ablation studies on various combinations of active and inactive regions.
% In active regions with an audio modality, visual embeddings whether active or not can be utilized as negative pairs, as speaker identities in both regions are same. 
% As audio embeddings in non-active region contain irrelevant sounds for the speaker, such as silence or another speaker's talk, we may treat the audio feature in the non-active frame as an additional negative sample.
% Moreover, we can utilize all samples to increase the number of samples. However, above approaches degrade performances.
% We guess that it is not directly related to the scores to use various samples because our loss needs delicate selection of positive and negative pairs to deal with synchronization between multi-modalities. 



==> tex/intro_copy.tex <==
\section{Introduction}
\label{sec:intro}
%1. asd 설명 
In today's technologically driven world, where multimedia content and virtual communication dominate, the significance of detecting an active speaker has never been more pronounced. The ability to understand who is speaking is paramount to understanding conversations in context. The objective of Active Speaker Detection (ASD) is to determine the active speaker in every video frame. ASD is frequently employed as a preliminary process for various speech-related tasks, including audio-visual speech recognition~\cite{afouras2018deep}, speech separation~\cite{owens2018audio,afouras2018conversation}, and speaker diarization~\cite{chung2019said,chung2020spot}.
% Figure 1
\captionsetup[figure]{font=small}
\begin{figure}[t!]
\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=7.5cm]{figures/graph3.pdf}}
\end{minipage}
\caption{Comparison of performances on the validation set of AVA-ActiveSpeaker dataset~\cite{roth2020ava}. Using our TalkNCE loss, three models~\cite{talknet, lightASD, loconet} attain performance increases. Specifically, when combined with LoCoNet~\cite{loconet}, our method achieves a state-of-the-art result.}
\label{fig1}
\end{figure}

%https://docs.google.com/spreadsheets/d/1AX7ry-eaIvJje7F6TgT3080XCpDNpLpo9LFcSFLzbY4/edit#gid=0

%2. temporal modeling의 구분 short long
Determination of whether an individual is actively speaking or not is a challenging task, thus requiring an effective integration both audio and visual information.
Recent studies~\cite{alcazar2020active,alcazar2021maas} suggest that ASD in real-world scenarios necessitates the following key elements: (1) The integration of audio-visual information for each speaker, (2) The inclusion of contextual information to capture inter-speaker relationships, and (3) The incorporation of temporal modeling to exploit long-term relationships within natural conversations. 
To address these specific requirements, ASD model architectures aim to create effective audio-visual features and comprehensively analyze these features over longer periods to capture crucial temporal information.
From the features obtained by proper modality-specific encoders, audio-visual fusion makes both information interactive. 
Cross-attention~\cite{talknet, loconet, jiang2023target} is employed for fusion by relating each visual stream with synchronized audio streams. After two features attend to each other, self-attention~\cite{talknet, loconet} or RNN-based architectures~\cite{lightASD, lwt} are mainly exploited to track the facial movements and lip motions for at least an utterance duration.  
The above approaches are suggested to take advantage of the complementary information of both modalities. 
However, there has been limited effort directed towards improving the individual modal features prior to the fusion stage. 
In this paper, we focus on the importance of supervision for encouraging feature extractor to learn audio-visual correspondence by contrastive learning, which is not widely discussed in other ASD methods.
%audio-visual fusion과 temporal modeling 모두 audio-visual correspondence를 잘 학습한 강력한 feature extractor와 함께 있을 때 최고의 효과를 가져올 수 있다.
%In this work, we propose a method which encourages the modality-specific encoder to incorporate the information from another modality by contrastive learning.}
%for bringing uni-modal features together into a common latent space,



% contrastive learning in ASD:
% RETHINKING AUDIO-VISUAL SYNCHRONIZATION FOR ACTIVE SPEAKER DETECTION: not on the loss side... augmentation of non-active samples
% Look Who's Talking: pretrained syncnet as an encoder + backend classifier
% SyncNet (prof's paper):
Contrastive learning is commonly exploited to enable the model to learn useful representations by training a model to distinguish between relevant and irrelevant data samples.
For multi-modal tasks~\cite{wuerkaixi2022rethinking}, a contrastive learning loss function highly depending on Noise-Contrastive Estimation (NCE)~\cite{gutmann2012noise} named InfoNCE~\cite{oord2018representation} can be used. 
To learn the natural correspondence of audio and video, a pair of synchronized audio and video is considered as positive, and the pair which is not in sync is considered as negative~\cite{chung2017out,chung2020perfect}.



%In this paper, we focus on the importance of supervision which is overlooked by other ASD methods, in contrast to the concentration afforded to the network architecture.
To this end, we devise the TalkNCE loss, a novel contrastive loss that provides appropriate supervision for the ASD task.
% to learn audio-visual correspondence which is essential for the ASD task. 
The loss acts on audio and visual features in a frame-wise manner rather than a sample-wise or chunk-wise one so that the loss enjoys a rich pool of negative samples by taking the maximum number of frames available.
Furthermore, considering the characteristics of the ASD task, the proposed loss is computed exclusively on the active speaking section where the audio and visual inputs are perfectly synchronized.
Trained with the TalkNCE loss, the encoders can focus more on details, especially audio-visual alignment, and enhance the effect of further stages denoted in Fig.~\ref{fig2}.
In contrast to the self-supervised contrastive learning approach for ASD~\cite{lwt} which adopts a two-stage training strategy, the model in our approach is trained using our loss jointly with the existing loss function in an end-to-end manner.
% \cite{lwt} used Multi-Way Matching (MWM) loss~\cite{perfectmatch2018, perfectmatch2020} for pre-training of the feature extractor, which is similar to our loss in terms of matching the synchronized audio-visual embedding pairs. 
% However, 
% In addition, \cite{lwt} froze the feature extractor to train the back-end classifier. In contrast, our model takes a multi-task learning strategy for enhancing the features as well as the optimization of the whole network for the main task. Moreover, we utilize all available frames in the video.
In the end, we demonstrate that the TalkNCE loss has generalizability as it brings performance gain when applied to existing ASD frameworks via extensive experiments indicated in Fig.~\ref{fig1}.
Especially combined with LoCoNet~\cite{loconet}, our method outperforms the previous state-of-the-art ASD methods on the AVA-ActiveSpeaker~\cite{roth2020ava} and ASW~\cite{lwt} datasets.

% 기존의 방법들은 feature extractor의 역할 간과 / model architecture 디자인에서 벗어나 supervision에 집중.
% audio-visual fusion과 temporal modeling 모두 audio-visual correspondence를 잘 학습한 강력한 feature extractor와 함께 있을 때 최고의 효과를 가져올 수 있다.
% network-agnostic / model-agnostic => generalization
% positive/negative sample을 구성하는 방법
% 2-stage 말고 e2e로 학습 가능.

Our contributions can be summarized as follows:
(1) We propose TalkNCE loss, a novel contrastive loss for ASD that enforces the model to exploit information from the synchronization and alignment of audio and visual streams. 
(2) The proposed loss can be plugged into multiple existing ASD frameworks and the additional supervision imposed by the loss improves the performances without any additional data.
(3) Our method outperforms previous state-of-the-art methods on the AVA-ActiveSpeaker dataset with a validation mAP of 95.5\%. 



% Nowadays, approaches to temporal information can be divided into long-term and short-term methods. 
% For humans, a few frames are not enough to guess who is speaking. 
% Looking at people for a long time can enhance performances drastically as in \cite{asc, EASEE, maas,asdnet, talknet, lightASD, loconet}. 
% Moreover, the judicious utilization of contextual cues, gleaned from the postures and gestures of co-present individuals within the shared scene, conveys a discernible advantage to the task. 
%referring to other people in the same scene by watching their poses and movements is beneficial to the task. 
% While \cite{EASEE, asdnet, maas} used only a single frame which inherently fail to encapsulate the full spectrum of pertinent details regarding alternate speakers, \cite{loconet} suggested short-term modeling for inter-speaker analysis using multiple frames.
% The utilization of audio input offers insights beyond mere speaker identity attributes, capturing synchronizations between audio and visual modalities.  
% Hence, adjusting both modalities bears significant pertinence in ASD tasks. 
% The most representative method is cross-attention~\cite{talknet, loconet} because it can align audio and visual streams along the time axis. Furthermore, a recent model~\cite{lightASD} proved that a simple element-wise addition is also an effective way of fusing audio-visual embedding pairs.

%4. 우리 거 좋은점?/
% While the potential benefits of both modalities are acknowledged, it is notable that the audio modality remains comparatively underutilized in scenarios including multiple faces within the frame~\cite{lightASD}. However, to cope with challenging cases such as lip occlusions, profiles, and small faces, the model should be accessible to information from audio.
% In this work, we propose a novel loss, named TalkSync loss, to encourage the model to learn the relations between synchronized audio and visual streams in temporal aspects. To the best of our knowledge, this is the first approach to deal with audio and visual embeddings to establish congruence within the multi-modal embedding spaces before feeding into audio-visual fusion for ASD predictions. Different from 0.2s receptive field in \cite{lwt}, our loss enjoys a rich pool of negative samples by taking advantage of the maximum number of frames available. As it is applied at the frame level, the model can catch details successfully. Moreover, our model is effectively optimized by simultaneously training the audio and visual encoder with the back-end modules. 

% Our contributions can be summarized as follows:
% (1) We propose a novel contrastive loss for ASD which enforces the model to exploit information from the synchronization of audio and visual streams. 
% (2) Our loss can be plugged-in for multiple other models and enhance their performances, as extra labeling or pre-processing of data are not required.
% (3) we achieved state-of-the-art results on the AVA-ActiveSpeaker dataset with a validation mAP of 95.5\% which is the most credible ASD dataset.



%Besides the improvement of the scores, training speed is accelerated by 1.5x in the case of TalkNet.



==> tex/method_copy.tex <==
\section{Method}
\label{sec:method}

\subsection{Preliminaries}
\label{ssec:method_prelim}

%
\begin{figure*}[t!]
\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=17cm]{figures/asd_arch_final_real.pdf}}
\end{minipage}
\caption{General framework for the active speaker detection task. Our loss is applied to the audio and visual embedding before the fusion. $\bigotimes$ denotes the concatenation of two features along the temporal dimension.}
\label{fig2}
%
\end{figure*}

This section describes the general ASD framework widely used in the literature~\cite{roth2020ava, talknet, lightASD, loconet, asc}.
ASD framework usually consists of feature extractors, audio-visual fusion, and temporal modeling, as shown in Fig~\ref{fig2}. 
For the input video frames containing $n_s$ speakers in the scene, every face is detected, cropped, stacked, and transformed to grayscale images $\mathbf{x}_v \in \mathbbm{R}^{n_s \times T \times H \times W}$, where $T$ denotes the number of frames and $H$ and $W$ denote the resolution. 
The corresponding audio waveform is transformed into mel-spectrogram $\mathbf{x}_a\in \mathbbm{R}^{4T \times C_{mel}}$ which indicates time and frequency. The frame length of $\mathbf{x}_a$ is intentionally set to 4 times of $T$ by adjusting hop length of Short-Time Fourier Transform (STFT).
Audio encoder $E_a(\cdot)$ and visual encoder $E_v(\cdot)$ encode inputs into $C$-dimensional frame-level audio and visual embeddings respectively, denoted as follows: 
\begin{equation}
\begin{split}
    & \mathbf{e}_a=E_a (\mathbf{x}_a),\quad \mathbf{e}_a \in \mathbbm{R}^{T \times C} \\
    & \mathbf{e}_v=E_a (\mathbf{x}_v),\quad \mathbf{e}_v \in \mathbbm{R}^{n_s \times T \times C}.
\end{split}
\end{equation}
To integrate the information between two modalities, two features are fed into an audio-visual fusion module. 
Note that before being fed into the fusion module, $\mathbf{e}_a$ is repeated for $n_s$ times to match the shape with the shape of $\mathbf{e}_v$. 
Except for GNN-based methods~\cite{EASEE, spell}, many recent methods such as TalkNet~\cite{talknet} and LoCoNet~\cite{loconet} utilize cross-attention layers for multi-modal fusion. 
By cross-attention mechanism, audio embedding could properly correspond to a related speaker along the time axis considering visual information.
Then the attention-weighted features $\mathbf{f}_a$ and $\mathbf{f}_v$ are concatenated to make the fused audio-visual features $\mathbf{f}_{av}$.

%%%% 3) Temporal modeling
Finally, several works~\cite{talknet, loconet, lightASD, EASEE, spell} employ a temporal modeling module by utilizing longer context to accurately predict the active speaker. 
Especially, LoCoNet~\cite{loconet} utilizes a combination of self-attention for a long-term intra-speaker analysis and convolutional layers to take account of short-term inter-speaker contexts at the same time. Besides, self-attention modules, a Gated Recurrent Unit (GRU), a Long Short-Term Memory (LSTM), and a Bidirectional LSTM (BiLSTM) are frequently exploited for temporal modeling.



%Feature extractor includes audio encoder $\psi_a$ and visual encoder $\psi_v$. Outputs of the encoders, which are $e_a = \psi_a (X_a)$ and $e_v = \psi_v (X_v)$, are combined through audio-visual fusion. Audio-visual feature $\mathbf{f}_{av}$ goes through temporal modeling to emit predictions. 
%%%% 1) Feature extractor
 %The corresponding audio signal is transformed into mel-spectrogram $X_a \in \mathbb{R}^{4T*C_m}$. $X_a$ is fed to audio encoder $\psi_a$ and becomes frame-level audio embedding $e_a \in \mathbb{R}^{T \times C_a}$. $T$ denotes the number of video frames, and the mel-spectrogram is extracted to have $4T$ time frames.
%For $n_s$ speakers in the scene, the face-crop images are stacked to make $X_v \in \mathbb{R}^{n_s \times T \times H \times W}$. Input images are in gray-scale. $X_v$ goes into visual encoder $\psi_v$ to yield a frame-level visual embedding $e_v \in \mathbb{R}^{n_s \times T \times C_v}$. 
%Before feeding to the cross-attention module, $e_a$ is repeated for $n_s$ times to match the shape of $e_a$ and $e_v$.
%%%% 2) A-V fusion

%Fusion of the embeddings from two modalities has a high impact on performance.
%Except for the models based on graph neural networks~\cite{EASEE, spell}, TalkNet~\cite{talknet} and several models including our baseline~\cite{loconet} used cross-attention layers for audio-visual fusion. By cross-attention, audio embedding could be matched to a proper person along the time axis given visual information. 

%\sy{Besides temporal modeling, incorporating audio-visual embedding is another factor that also highly impacts performance. Except for the models based on graph neural networks~\cite{EASEE, spell},~\cite{talknet} and several models including our model used cross-attention layers for audio-visual fusion. By cross-attention, audio embedding could be matched to a proper person along the time axis given visual information. }
%Recently, \cite{lightASD} proved that a simple element-wise addition would be a way of multi-modal fusion. 
%However, there is a case with substantial amounts of parameters when addition degrades performances. 
%Our model focuses on temporal modeling and naturally model size is not smaller compared to \cite{lightASD} which utilized only 1 million parameters.

%\sy{Our baseline model~\cite{loconet} utilizes both long-term intra-speaker context and short-term inter-speaker context. Seeking an active speaker is difficult when several people talks each other, thereby it is necessary to look the target person for long time and other people for at least several frames. LoCoNet~\cite{loconet} appeared recently and achieved a successful score for AVA-ActiveSpeaker~\cite{roth2020ava} validation set which is the most prominent dataset in ASD. }



%
% \begin{figure}[htb]
% \begin{minipage}[b]{1.0\linewidth}
%   \centering
%   \centerline{\includegraphics[width=8.5cm]{talknet.png}}
% \end{minipage}
% \caption{Our loss is applied for the audio and visual embedding before cross-attention in TalkNet~\cite{talknet}.}
% \label{fig:res}
% %
% \end{figure}


\subsection{TalkNCE Loss}
\label{ssec:method_loss}

A training objective typically used in the ASD task~\cite{roth2020ava, talknet, lightASD, loconet, asc} can be represented as follows: \jyj{(see comment.)}
\begin{equation} 
\label{eq2}
 \mathcal{L}_{model} = \mathcal{L}_{av} + \lambda_a \cdot \mathcal{L}_a + \lambda_v \cdot \mathcal{L}_v, 
\end{equation}
where $\mathcal{L}_{av}$ denotes the cross-entropy loss between the ground-truth labels and the final frame-level predictions after temporal modeling. 
$\mathcal{L}_a$ and $\mathcal{L}_v$ are auxiliary cross-entropy losses that are computed with uni-modal features $\mathbf{f}_a$ and $\mathbf{f}_v$ to make the model utilize both modalities in a balanced manner.
% ~\cite{roth2020ava, asc, loconet}

In addition to the cross-entropy loss, we introduce TalkNCE loss, a talk-aware contrastive loss that provides supervision for models to learn audio-visual correspondence.\jyj{(see comment.)}
% In addition to this, we introduce a new loss function, named TalkSync loss, which is a contrastive loss to assist an audio-visual fusion stage for each time step. 
%The attention map from cross-attention layers showed that the information from the audio was not completely utilized for the task. 
The proposed loss brings audio-visual embedding pairs closer if they come from the same video frame and makes them push each other away otherwise. 
This encourages the encoders to detect salient information regarding audio-visual synchronization and to concentrate on fine details including frame-level correlation between audio and visual modalities.

% zhang2019multi, wuerkaixi2022rethinking: includes whole segments
% lwt, chung2017out: requires pre-training of encoders
Previous papers~\cite{zhang2019multi, lwt, wuerkaixi2022rethinking, chung2017out} include cross-modal contrastive learning for ASD task. However, different from our method, their approaches either require pre-training of the feature extractor or include non-active segments in the calculation of the contrastive loss. 

Our new loss optimizes frame-level matching between paired audio and visual streams as denoted in Fig~\ref{fig:res}. 
Given the audio and visual embeddings $\mathbf{e}_a$ and $\mathbf{e}_v$, the active speaking regions are extracted using the original ASD labels.
Let $T_{act}$ be the length of active speaking region and $\{\mathbf{e}_{a,i}\}_{i \in \{1,...,T_{act}\}}$, $\{\mathbf{e}_{v,i}\}_{i \in \{1,...,T_{act}\}}$ be the frame-level audio and visual embeddings for the active speaking region.
Then the TalkNCE loss $\mathcal{L}_{TalkNCE}$ can be represented as follows:

\begin{equation}
\label{eq4}
    \mathcal{L}_{TalkNCE} = -\cfrac{1}{T_{act}} \sum_{i=1}^{T_{act}} \log \cfrac{\exp(s_{i,i} \slash \tau)}{\sum_{j=1}^{T_{act}} \mathbbm{1}_{[j \neq i]} \exp(s_{i,j} \slash \tau)},
\end{equation}
where $s_{i,j} = \norm{\mathbf{e}_{v,i}}^T \norm{\mathbf{e}_{a,i}}$ and $\tau$ represents a temperature constant fixed to 1. 
Summing up the TalkNCE loss and the original ASD loss, the final training objective used in this paper can be formulated as follows:\jyj{(see comment.)}

\begin{equation}
\label{eq5}
\begin{split}
 %  \mathcal{L} = &\, \mathcal{L}_{av} + \lambda_a \cdot \mathcal{L}_a + \lambda_v \cdot \mathcal{L}_v & +\lambda_{TalkNCE} \cdot \mathcal{L}_{TalkNCE},
   \mathcal{L} = \mathcal{L}_{model} +\lambda \cdot \mathcal{L}_{TalkNCE},
\end{split}
\end{equation}
where $\lambda$ is the weight value of TalkNCE loss.

% We introduce a new loss term $\mathcal{L}_{TalkSync}$ as in Eq~\ref{eq4}. $\lambda_a$, $\lambda_v$, and $\lambda_{TalkSync}$ are the weight values of audio auxiliary loss, visual auxiliary loss, and TalkSync loss, respectively.


% Details are as follows: 1) In a training step, using given original labels, extract active speaking regions for $e_v$ and corresponding $e_a$. 
% 2) For extracted $e_a$ and $e_v$, a similarity matrix $M \in \mathbb{R}^{T\times T}$ is calculated by matrix-multiplication of $e_a$ and transposed visual features in Eq~\ref{eq3}. 
% 3) Elements on the diagonal axis are similarity values of a positive pair because audio and visual features should be matched denoting the same phoneme. 
% 4) Divide the similarity matrix into positive and negative pairs, which are the diagonal axis and the rest respectively. 
% 5) Reorganize the table by putting the positive pair on the first column and negative pairs on the remaining $T-1$ columns. 
% 6) Compute cross-entropy loss between positive and negative pairs as \cite{silva2020exploring}. $M_{i1}$ denotes the first frame of positive pairs and $M_{it}$ is the rest of the negative frames which do not belong to the diagonal axis as in Eq~\ref{eq4}.

% \cite{lwt} used Multi-Way Matching (MWM) loss~\cite{perfectmatch2018, perfectmatch2020} for pre-training of the feature extractor, which is similar to our loss in terms of matching the synchronized audio-visual embedding pairs. 
% However, 
% In addition, \cite{lwt} froze the feature extractor to train the back-end classifier. In contrast, our model takes a multi-task learning strategy for enhancing the features as well as the optimization of the whole network for the main task. Moreover, we utilize all available frames in the video.


%as our feature encoder consumes inputs with variable lengths.

%Cross-attention is good enough to relate audio-visual embedding for each time step proved in high scores 
%but when we see the attention map after audio-visual cross-attention layers, audio information is not fully used for the task. 
%Therefore, we applied TalkSync loss for the outputs of the audio encoder and the visual encoder to make both outputs integrate with each other at the frame level unit. As in Fig 2, right before entering to cross-attention layers, our loss is attached to bring appropriate audio-visual embedding pairs closer. 




